Domain Adaptation for Code Model-based Unit Test Case Generation

Recently, deep learning-based test case generation approaches have been proposed to automate the generation of unit test cases. In this study, we leverage Transformer-based code models to generate unit tests with the help of Domain Adaptation (DA) at a project level. Specifically, we use CodeT5, a relatively small language model trained on source code data, and fine-tune it on the test generation task. Then, we apply domain adaptation to each target project data to learn project-specific knowledge (project-level DA). We use the Methods2test dataset to fine-tune CodeT5 for the test generation task and the Defects4j dataset for project-level domain adaptation and evaluation. We compare our approach with (a) CodeT5 fine-tuned on the test generation without DA, (b) the A3Test tool, and (c) GPT-4 on five projects from the Defects4j dataset. The results show that tests generated using DA can increase the line coverage by 18.62%, 19.88%, and 18.02% and mutation score by 16.45%, 16.01%, and 12.99% compared to the above (a), (b), and (c) baselines, respectively. The overall results show consistent improvements in metrics such as parse rate, compile rate, BLEU, and CodeBLEU. In addition, we show that our approach can be seen as a complementary solution alongside existing search-based test generation tools such as EvoSuite, to increase the overall coverage and mutation scores with an average of 34.42% and 6.8%, for line coverage and mutation score, respectively.

==> response.tex <==
\section*{Response to Reviewers}
We are thankful for the valuable feedback provided by the reviewers and the chance to improve our paper.
In response to your insightful comments, we have updated our manuscript.
Modification includes adding necessary details and analyses, clarifying ambiguous sections, and strengthening the study.
The revisions follow the sequence outlined in the meta-review, and we have diligently addressed each detailed comment from the reviewers to the best of our ability.
We refer to specific locations of each change using \citeresp{X-XX}. 
You can click \textbf{\textcolor{blue}{X}} (``on page \textbf{\textcolor{blue}{X}}'') to jump to the modified location.

\subsection*{Point 1: Empirically compare with at least one of the recent LLM-based test generation techniques (e.g., CodeMOSA, ChatTester, or TestPilot).} 
\review{Reviewer \#1: Compare with recent closely relevant work, including CodaMOSA, TestPilot, ChatTester, and TeCo.}

\noindent Thank you for the suggestion! We explored all suggested test generation tools, but unfortunately, none could be applied in our case! Regarding \emph{TestPilot}, firstly, their proposed method relies on an API exploration component, taking the target npm package and using dynamic analysis to identify the functions and their definitions, access paths from the main module, parameters with type information, etc. Secondly, their documentation miner component relies on API usage examples extracted from npm packages. However, most of our target packages' API documents (JavaDoc) did not provide examples of API usage. 
\emph{CodaMOSA}, the next suggested tool, is based on \emph{Pynguin}, an SBST tool for Python code, not Java, which is the language of our dataset samples. The next tool,\emph{TeCo}, focuses on a different task, test completion, instead of whole unit test case generation. 
We tried using \emph{ChatTester} as it was the only LLM-based approach that shares the same target language and task as ours. However, the tool did not work on most projects we used for the evaluation. The main reason was that their data-pair collection component failed to extract the unit test cases and the focal methods. Due to this reason, their component was only able to extract 1.7K data instances from 185 projects. Out of the 5 Defects4j projects we use for evaluation, the tool could only extract 20 instance pairs from one project and none from the other four, which is insufficient for proper comparison.
We did not modify their code to make it applicable since it required much overhead due to their shared repositories lacking documentation, data, and use case examples.
However, since \emph{ChatTester} is an improvement over the \emph{GPT} model by applying iterative-styled prompt engineering, we argue that our \emph{GPT-4} baseline serves as an acceptable replacement for this tool, as the focus of our study is not on different prompt engineering strategies. 
% \song{say you will mention this in the threats to validity}\jiho{Sure.}
We will mention these as our threats to validity in Section \ref{sec:threats}.

\noindent The content marked with\citerespexp{1-1} is the location of the discussion.

\subsection*{Point 2: Highlight your work's key novelty/contribution and compare it with other state-of-the-art work.} 
\review{Reviewer \#1: Clarify the study's core novelty and main contribution.}

\noindent The key novelty of this paper compared to existing test generation using pre-trained models is that we adopt two different levels of fine-tuning/domain adaptation (i.e., task-level and project-level) on a relatively smaller language model to outperform bigger language models, i.e., \emph{GPT-4}. To our knowledge, this idea has never been studied in the literature. Our results are also significant, as we could outperform the state-of-the-art LLM (\emph{GPT-4} with 1.76T parameters) with a much smaller model (\emph{CodeT5} with 220M)
% \song{do you have a reference for such a claim?}\jiho{This is a general claim I made observing the current trend of LLM. I will change the presentation.}
. In addition, our findings show that test case generation tasks rely more on fine-tuning with project/domain-specific data than only task-specific data, which has not been investigated. We added discussions to clarify these points in Section \ref{sec:intro}.

\noindent The content marked with \citerespexp{2-1} is the location of the change. \\

\noindent \review{Reviewer \#1: Include a detailed discussion of the closely relevant work.}

\noindent Thank you for the suggestion! We added the suggested relevant test generation studies in the Background Section \ref{sec:bg} as follows. 
Lemieux et al. \cite{lemieux2023codamosa} proposed \emph{CodaMOSA}, an SBST approach that leverages LLM for escaping the coverage plateau for Python code bases. Schafer et al. \cite{schafer2023empirical} proposed \emph{TestPilot}, a test cases generation approach that leverages LLM, usage examples mined from package documentation, and error logs for npm packages (JavaScript). Yuan et al. \cite{yuan2023no} proposed \emph{ChatTester}, which is an LLM-based test case generation model that exploits \emph{ChatGPT} and iterative generate-and-validate prompt engineering strategy with execution feedback. Nie et al. \cite{nie2023learning} proposed \emph{TeCo}, a deep encoder-decoder test completion model that learns different levels of code semantics and re-ranking by execution. A test completion model generates the following statement of a unit test case when the previous line and method under test are given as context.

\noindent The content marked with \citerespexp{2-2} is the location of the change. 

\subsection*{Point 3: Add mutation score analysis to all RQs.} 
\review{Reviewer \#1: Perform a more in-depth analysis of the mutation scores and include it for all RQs.}

\noindent Thank you for the insight to improve our paper. We have added the mutation score for the other RQs (RQ1--2) and the in-depth analysis. The discussions on the additional experiments can be found in Sections \ref{sec:rq2_result}.

\noindent The content marked with \citerespexp{3-1} is the location of the change. 

\section*{Other detailed comments.}
We also tried our best to address all the detailed comments from the reviews not included in the latter meta-reviews in the following sections. 

\subsection*{Point 1: The soundness or lacking discussion about the experimentation.}
\review{Reviewer \#1: Justify why extra context information is needed for each target line when applying domain adaptation.}

\noindent %A target line can be as simple as a return statement or adding two variables. 
The model needs more context to generate meaningful unit tests, such as the class name, method names, variable names, and the whole focal method. A single line would not provide enough information for a language model to generate meaningful unit tests, so we added the extra context. 
Note that our context design strictly follows the baseline work from the Methods2Test dataset, which we used for fine-tuning downstream tasks. To clarify this point, we have added more explanations in Section \ref{sec:da_approach}. 

\noindent The content marked with \citerespexp{a-1} is the location of the change. \\

\noindent \review{Reviewer \#1: Justify how selecting 20\% of each project's unique tests as an evaluation set avoids leakage issues.}

\noindent Since similar test cases are distributed in both train and test sets, this could be seen as an unfair or leakage in information. However, we argue that similar test cases shouldn't necessarily be considered as information leakage since a similar test case that verifies different values for an assertion (two test cases that only differ from the values they check) could have been specifically designed to verify a particular control flow of a focal method. In addition, another indicator that the generated tests are different from the tests in the train set is that the generated tests cover new lines compared to the developer-written tests' line coverage. \\

\noindent \review{Reviewer \#2: Empirically investigate the effect of quality and quantity of initial test suite on the proposed approach.}

\noindent Thank you for the comment on an interesting future direction! If there are no test suites for a project for domain adaptation, the result is reported as RQ1. As suggested by the comment, we can assess the performance with different numbers of test cases and different levels of quality. However, this additional experiment must consider many design choices, e.g., different cut-off numbers of test cases and the test case quality metric (effectiveness, readability, test code quality, etc.). Therefore, we believe correctly addressing this suggestion is beyond this paper and would consider this idea for future work. \\

\noindent \review{Reviewer \#2 and \#3: Provide more details about the fine-tuning process applied in the study.}

\noindent The fine-tuning process optimizes the pre-trained model for the downstream task (e.g., test case generation), which many related studies on domain adaptation have adopted. In this work, we follow the same logic while adding a second level of domain adaptation based on project-specific data.
We use task-level fine-tuning because the CodeT5 model was not explicitly trained to generate unit test cases for focal methods. The dataset used to fine-tune testing-related downstream tasks is from a former study Methods2Test dataset. To fine-tune this, we followed the original CodeT5 model. Specifically, as suggested in their paper, we used the conditional code generation method. We revised the presentation in Section \ref{sec:noda_approach} to clarify the details applied to the fine-tuning process.

\noindent The content marked with \citerespexp{a-4} is the location of the change. \\

\noindent \review{Reviewer \#2: The authors have trained the model for a few more epochs for domain adaptation. Did they consider freezing some weights during such additional epochs to speed up convergence?}

\noindent As mentioned in the manuscript, we have tried this approach in our preliminary study. However, we didn't find any benefit in the model's performance. The best performance was achieved by fine-tuning all the layers, so we selected this method. 

\noindent The content marked with \citerespexp{a-5} is the location of the discussion. \\

\noindent \review{Reviewer \#2: Search-based approaches do not require training, which is a computation and time-consuming activity. The authors should acknowledge this when comparing the computation time of the two approaches (e.g., in the referred sentence).}

\noindent Thank you for the comment. We added this discussion to the referred sentence, as we did not compare the time exactly. However, we want to point out that the training cost is a one-time cost. For SBST, however, the search cost is ongoing per instance. Therefore, the cost of running SBST tools would be higher if the number of instances grows.

\noindent The content marked with \citerespexp{a-6} is the location of the change. \\

\noindent \review{Reviewer \#2 and \#3: Include compilability/executability of the generated tests.} 

\noindent Thank you for the suggestion! We also deem this as an interesting metric. We added the following metrics for the parse and compile rates in the paper. The explanation of the metrics can be found in Section \ref{sec:metrics}. Additional experimental results and the analysis can be found in Section \ref{sec:evaluation}. \\

\noindent \review{Reviewer \#3: Justify the research's generalizability and external validity.}

\noindent We agree that the selected project can threaten this study's external validity. However, Defects4j is a well-known and widely used dataset with quality unit test cases. Using a limited number of projects is mainly due to the considerable resource cost of calculating the test adequacy metrics. Due to the same reason, some of the previous studies that evaluate test adequacy metrics (i.e., line coverage or mutation score) on test or test oracle generation also experimented with a small number of projects like us, e.g., TOGA \cite{dinella2022toga} and A3Test \cite{alagarsamy2023a3test}. Also, it is worth noting that running GPT-4 per each extra project is very costly, hindering the experiments' size. We added these discussions as external threats to validity for clarification in Section \ref{sec:threats}.

\noindent The content marked with \citerespexp{a-8} is the location of the change. \\

\noindent \review{Reviewer \#3: The experimental setup is not complete and solid. The first research question, 'Can Transformer-based code models generate high-quality test cases,' seems to be addressed with domain adaptation validation conducted only on the Defects4j dataset using the CodeT5 model. It is insufficient to substantiate the performance of the results for RQ1, as well as for RQ2.}

\noindent RQ1 examines the ability of \emph{CodeT5} to generate test cases by fine-tuning task-specific training data without domain adaptation. RQ2 examines the ability of project-level domain adaptation and compares their efficacy on current state-of-the-art baselines. We agree that RQ1 seems overstating. We have revised the RQ1 to ``How effective is \emph{CodeT5} in generating unit test cases without domain adaptation?''.\\


\subsection*{Point 2: Presentation}
\review{Reviewer \#2: The text contains a few repetitions that could be avoided.}

\noindent Thank you for the comment. We have done multiple rounds of proofreading on the manuscript to reduce duplicate discussions and improve language presentation. \\ 

\noindent \review{Reviewer \#2: Tone down the language where authors consider the BLEU and CodeBLEU metrics as ``poorly relevant''.}

\noindent Thank you for the suggestion. We will tone down on the language as it could reflect different aspects of the generations, i.e., readability and similarity.

\noindent The content marked with \citerespexp{b-2} is the location of the change. \\

\noindent \review{Reviewer \#2: Tone down the language where authors mention: ``However, in source code, identifier numbers can be interchangeably named''}

\noindent Thank you for the suggestion! We will tone down the referred sentence to ``However, there is more than one way of naming an identifier in source code.''.

\noindent The content marked with \citerespexp{b-3} is the location of the change. \\
